Knowledge Fusion By Evolving Weights of Language Models

Fine-tuning pre-trained language models, particularly large language models, demands extensive computing resources and can result in varying performance outcomes across different domains and datasets. This paper examines the approach of integrating multiple models from diverse training scenarios into a unified model. This unified model excels across various data domains and exhibits the ability to generalize well on out-of-domain data. We propose a knowledge fusion method named Evolver, inspired by evolutionary algorithms, which does not need further training or additional training data. Specifically, our method involves aggregating the weights of different language models into a population and subsequently generating offspring models through mutation and crossover operations. These offspring models are then evaluated against their parents, allowing for the preservation of those models that show enhanced performance on development datasets. Importantly, our model evolving strategy can be seamlessly integrated with existing model merging frameworks, offering a versatile tool for model enhancement. Experimental results on mainstream language models (i.e., encoder-only, decoder-only, encoder-decoder) reveal that Evolver outperforms previous state-of-the-art models by large margins. The code is publicly available at {https://github.com/duguodong7/model-evolution}.

==> evonlp/resources/ablation1.tex <==
% \documentclass{article}
% \usepackage{graphicx}
% \usepackage{subcaption}
\begin{figure}[h]
\vspace{-0.1cm}
\begin{minipage}{0.48\textwidth} % Left minipage for subfigures
\centering
\includegraphics[width=\textwidth]{evonlp/resources/figs/iteration.pdf}
\caption{In-domain score of model evolution on emotion dataset with all domain specific models. The results on both the development and test dataset are displayed.}
\label{fig:combined}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth} % Right minipage for a single image
\centering
% \vspace{0.48cm} % Adjust this value to move the image down
\includegraphics[width=\textwidth]{evonlp/resources/figs/diff_afa.pdf}
\caption{The improvement of \textit{regmean-evolver} with different scale $\alpha$ on emotion dataset when evolving all domain specific models. $*$ means the result of \textit{simple} and \textit{evolver}.}
\label{fig:diff_afa}
\end{minipage}
% \vspace{-0.3cm}
\end{figure}


% \begin{figure}
%     \begin{minipage}{0.47\textwidth} % Left minipage for subfigures
%         \begin{subfigure}{0.48\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{evonlp/resources/figs/roberta.pdf}
%             \caption{Left Subfigure 1}
%             \label{fig:left-subfig1}
%         \end{subfigure}
%         \begin{subfigure}{0.48\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{evonlp/resources/figs/distilbert.pdf}
%             \caption{Left Subfigure 2}
%             \label{fig:left-subfig2}
%         \end{subfigure}
%         \label{fig:iteration}
%         \caption{left Figure}
%     \end{minipage}
%     \begin{minipage}{0.53\textwidth} % Right minipage for a single image
%         \centering
%         \includegraphics[width=\textwidth]{evonlp/resources/figs/diff_afa.pdf}
%         \caption{Right Figure}
%         \label{fig:right-fig}
%     \end{minipage}
%     % \caption{Main Figure with Two Subfigures on the Left and One Figure on the Right}
%     % \label{fig:main-figure}
% \end{figure}




==> evonlp/resources/comparision.tex <==
\begin{table*}[t]
\vspace{-1cm}
\centering
\scalebox{0.7}{
\begin{tabular}{ccccccc}
\toprule
  & Ensemble  & Model Merging & Multitask Learning & Federated Learning & Model Soups  & \textbf{Model Evolution (ours)}  \\
\midrule
Retraining & \ding{55} & \ding{55} & \ding{51} &\ding{51} & \ding{55} & \ding{55} \\
High Memory Cost & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55}  \\
Round(s) & Single & Single & Single & Multiple & Greedy & Greedy \\
Data & No & A Few Examples &Train Datasets & Private & Dev Datasets & Dev Datasets \\
Key Technique &  Inference & Matrices Computing & Distribution & Back-Propagation & Search &  Evolution \\
Peak GPU Memory &\ding{55} & \ding{51}  & \ding{51} & \ding{51}  &\ding{55} & \ding{55}  \\
\bottomrule
\end{tabular}}
\caption{Comparison of different knowledge fusion methods. Dev datasets means development dataset for validation. Round means the number of times the models are edited when implementing a certain knowledge fusion method. The key technique highlights the difference between knowledge fusion methods. Peak GPU memory is considered low for search or evolution step since only inference is needed. We do not include simple weight averaging method into model merging here.}
\label{tab: comparison}
\vspace{-0.7cm}
\end{table*}



==> evonlp/resources/glue_result_fig.tex <==
\begin{figure}[h]
\vspace{-0.2cm}
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{evonlp/resources/figs/glue_niid.pdf}
    \caption{Result of model evolution on non-i.i.d. partitions of GLUE benchmark datasets.}
    \label{fig3:glue-niid}
  \end{minipage}
  \hfill  % This adds a horizontal space.
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{evonlp/resources/figs/glue_difftask.pdf}
    \caption{Result of model evolution across different pairwise tasks on GLUE benchmark.}
    \label{fig4:glue-diff-task} 
  \end{minipage}
\end{figure}
\vspace{-0.5cm}


==> evonlp/resources/hotmap.tex <==
\begin{figure}
% \hspace{-0.2cm}
% ,height=0.4\textwidth
\centering
\includegraphics[width=0.49\textwidth]{evonlp/resources/figs/hotmap.pdf}
\caption{The average performance of merged T5 model on MRPC and STSB test dataset. By observing the density and distribution range of the contour lines, it is evident that our evolver method performs better. Additionally, previous methods typically utilize a uniform scale across different task vectors, whereas the evolved model exhibits a preference for varying scales determined through iterative evolution rounds.}
\label{fig:hotmap}
% \vspace{-0.2cm}
\end{figure}

==> evonlp/resources/in_domain_all.tex <==
\begin{table*}[h]
\centering
\scalebox{0.75}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
& \multicolumn{1}{c}{Encoder-Decoder} & \multicolumn{3}{c}{Encoder-only} & \multicolumn{2}{c}{Decoder-only} \\
\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7} 
Method & T5-base &
\begin{tabular}[c]{@{}c@{}}RoBERTa-base \\ Same / Diff Head Init.\end{tabular} &
\begin{tabular}[c]{@{}c@{}}DistilBERT-base \\ Same / Diff Head Init.\end{tabular} &
\begin{tabular}[c]{@{}c@{}}DeBERTa-large \\ Same / Diff Head Init.\end{tabular} & 
 GPT2 & MiniCPM \\
\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7} 
Avg. $f_{1..\textsc{N}}$  & 32.07 & 26.08  & 24.55 & 27.68 & 23.35 & 35.12 \\
Best. $f_{1..\textsc{N}}$  & 34.08 & 29.27  & 29.91 & 31.93 & 26.76 & 37.23 \\
Ensemble         & 33.95 & 38.77 / 27.73 & 26.51 / 25.43 & 29.88 / 29.27 & 26.82 & 37.05 \\
Greedy Soup      & 34.10 & 30.34  & 30.11  & 31.93 & 26.76 & 37.31 \\ \midrule
Simple           & 39.47 & 23.18  & 23.70  &  3.75 & 21.54 & 42.44  \\
Evolver          & 41.25 & 33.27 / 30.04 & 28.95 / 26.29 & 23.90 / 21.55 & 23.41 & 44.76  \\ \midrule
Fisher           & 39.12 & 26.09 / 22.43 & 26.39 / 22.61 & 12.83 / 20.42 & 24.93 & \textbackslash  \\
Fisher\_Evolver  & 40.36 & 28.41 / 25.71 & 27.63 / 24.75 & 17.22 / 22.95 & 25.66 & \textbackslash \\ \midrule
RegMean          & 40.24 & 38.74 / 32.58 & 33.37 / 28.29 & 38.33 / 18.92 & 30.14 & \textbackslash  \\
RegMean\_Evolver   & 41.83 & 39.87 / 34.28  & 35.67 / 31.11 & 39.58 / 21.79 & 32.26 & \textbackslash  \\ \midrule
TIES           & 41.24 & 39.66 / 35.32  & 35.55 / 30.14 & 39.22/ 21.67 & 32.11 & 45.81 \\
\textbf{TIES\_Evolver}  & \textbf{43.16} & \textbf{41.33} / \textbf{37.42}  & \textbf{37.12} / \textbf{31.48} & \textbf{40.61} / \textbf{23.24} & \textbf{33.56} & \textbf{46.24} \\ \midrule
Domain-Specific  & 49.31 & 51.38         & 48.79         & 52.81   & 47.62 & 54.32 \\ 
MTL              & 48.98 & 47.73         & 45.23         & 51.77   & 44.31 & 52.14 \\
\bottomrule
\end{tabular}
}
\caption{\small{In-domain performance when merging emotion classification models. The initial population are all 5 domain specific models or pairwise models. Simple, Fisher, RegMean and TIES are model merging algorithms for comparison. $\textbackslash$ indicates the method can not been conducted due to high GPU cost. \textbf{Bold} numbers indicate the best performance across different model merging algorithms. All the results we reported are averages of trials conducted with 5 different random seeds.}}
\label{tab:merge_all_in_domain}
\end{table*}



==> evonlp/resources/ood_all.tex <==
\begin{table*}[h]
\centering
\scalebox{0.75}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
& \multicolumn{1}{c}{Encoder-Decoder} & \multicolumn{3}{c}{Encoder-only} & \multicolumn{2}{c}{Decoder-only} \\
\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7} 
% \begin{tabular}[c]{@{}l@{}}Model ($\rightarrow$) \\ Method ($\downarrow$) \end{tabular} &
Method & T5-base &
\begin{tabular}[c]{@{}c@{}}RoBERTa-base \\ Same / Diff Head Init.\end{tabular} &
\begin{tabular}[c]{@{}c@{}}DistilBERT-base \\ Same / Diff Head Init.\end{tabular} &
\begin{tabular}[c]{@{}c@{}}DeBERTa-large \\ Same / Diff Head Init.\end{tabular} & 
 GPT2 & MiniCPM \\
\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7} 
Avg. $f_{1..\textsc{N}}$  & 30.12 & 20.92     & 19.69        & 21.17   & 18.63 & 35.24    \\
Best. $f_{1..\textsc{N}}$ & 37.41 & 29.46     & 29.55        & 31.07   & 27.88 & 38.93   \\
Ensemble         & 27.92 & 11.36 / 10.90 & 9.60 / 9.19   & 11.09 / 9.26   & 8.77 & 29.54 \\ 
Greedy Soup      & 15.42   & 13.43     & 15.26        & 4.67    & 11.61 & 31.70    \\ \midrule
Simple           & 38.61   & 11.56   & 13.21   &  0.24  & 10.25 & 40.21  \\
Evolver          & 39.26   & 17.53 / 17.16 & 19.02 / 18.42 &  13.33 / 12.78  & 15.87 & 42.48 \\ \midrule
Fisher           & 37.72   & 16.21 / 14.28 & 17.77 / 15.69   & 5.57 / 27.61   &  15.16 & \textbackslash \\
Fisher\_Evolver  & 38.87   & 16.98 / 15.44 & 18.85 / 17.36   & 15.46 / \textbf{30.41}  &  16.34 & \textbackslash \\ \midrule
RegMean          & 39.46   & 21.09 / 14.12 & 18.97 / 16.21   & 15.92 / 4.88  & 20.33 & \textbackslash \\ 
RegMean\_Evolver & 41.13   & 23.41 / 16.45 & 21.44 / 18.31   & 18.49 / 11.27  & 22.07 & \textbackslash \\ \midrule
TIES             & 40.48   & 22.63 / 16.34 & 19.76 / 17.52   & 16.88 / 14.72  & 21.92 & 41.35 \\ 
\textbf{TIES\_Evolver}    & \textbf{42.53 }  & \textbf{24.11 / 19.02} & \textbf{22.64 / 19.06}   & \textbf{18.74} / 16.31  & \textbf{22.75} & \textbf{42.86} \\ \midrule
MTL      & 37.64  & 27.41      & 25.63        & 31.45       & 25.26  & 44.62   \\ 
\bottomrule
\end{tabular}
}
\caption{\small{Performance evaluation of model evolution in out-of-domain context.}}
\label{tab:merge_all_ood_emotion}
\end{table*}



==> evonlp/resources/overview.tex <==
\begin{figure}
\centering
\includegraphics[width=0.49\textwidth]{evonlp/resources/figs/fig1_final.pdf}
\caption{The key step in our proposed model evolution method is to aggregate models $f_{1..N}$ from various environments as a population and updating it through greedy evolutionary rounds.}
\label{fig:model-evolver-overview}
\end{figure}


==> evonlp/resources/pairwise_emotion.tex <==
\begin{table}[h]
\centering
\scalebox{0.75}{
\begin{tabular}{@{}c|cc|cc}
\toprule
Model & Simple & Evolver & TIES & \textbf{TIES\_Evolver} \\
\cmidrule(r){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
T5-base          & 38.82  & 40.21  & 46.35  & \textbf{47.92}  \\
RoBERTa-base     & 37.78  & 39.13  & 45.56  & \textbf{46.89}  \\
DistillBERT-base & 36.76  & 38.85  & 42.09  & \textbf{43.22}  \\
DeBERT-large     & 38.11  & 39.46  & 45.87  & \textbf{46.78}  \\
GPT2             & 36.33  & 38.25  & 41.85  & \textbf{42.62}  \\
MiniCPM          & 40.22  & 42.71  & 47.02  & \textbf{48.83}  \\
\bottomrule
\end{tabular}
}
\caption{\small{In-domain performance when merging pairwise domain-specific emotion classification models. All the results we reported are averages of 10 ($\mathcal{C}^2_5$) runs after paring models from a set of 5.}}
\label{tab:pairwise_emotion}
\end{table}
